On-The-Go Robot-to-Human Handovers with a Mobile Manipulator

Existing approaches to direct robot-to-human handovers are typically implemented on fixed-base robot arms, or on mobile manipulators that come to a full stop before performing the handover. We propose "on-the-go" handovers which permit a moving mobile manipulator to hand over an object to a human without stopping. The on-the-go handover motion is generated with a reactive controller that allows simultaneous control of the base and the arm. In a user study, human receivers subjectively assessed on-the-go handovers to be more efficient, predictable, natural, better timed and safer than handovers that implemented a "stop-and-deliver" behavior.

==> figures/boxplot.tex <==
% LTV-MPC CPU TIME COMPARISON
%     \begin{tikzpicture}
%     \begin{axis}[
%         boxplot/draw direction=y,
%         xtick={1,2,4,5},
%         xticklabels={MR, SR, MH, SH},
%         ymin = 0.75, ymax = 5.25,
%         ]
%         \addplot [solid, blue, mark=*, boxplot prepared={
%             lower whisker   =   3, 
%             lower quartile  =   4,
%             median          =   4, 
%             upper quartile  =   5,
%             upper whisker   =   5},
%         ] coordinates {};
        
%         \addplot [solid, red, mark=*, boxplot prepared={
%             lower whisker   =   1.5, 
%             lower quartile  =   3,
%             median          =   4, 
%             upper quartile  =   4,
%             upper whisker   =   5},
%         ] coordinates {(2, 1)};
        
%         \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
%             lower whisker   =   5, 
%             lower quartile  =   5,
%             median          =   5, 
%             upper quartile  =   5,
%             upper whisker   =   5},
%         ] coordinates {(4, 4)};
        
%         \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
%             lower whisker   =   2.5, 
%             lower quartile  =   4,
%             median          =   5, 
%             upper quartile  =   5,
%             upper whisker   =   5},
%         ] coordinates {(5, 2)};        
%     \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            name=mainplot,
            title=\textbf{Efficiency},
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            ytick={1,2,3,4,5},
            ymin = 0.75, ymax = 5.25,            
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   3, 
            lower quartile  =   4,
            median          =   4, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   1.5, 
            lower quartile  =   3,
            median          =   4, 
            upper quartile  =   4,
            upper whisker   =   5},
        ] coordinates {(2, 1)};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(4, 4)};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   2.5, 
            lower quartile  =   4,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(5, 2)};      
        
    \end{axis}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            name=secondplot,
            title=\textbf{Naturalness},
            at={(mainplot.north east)},
            xshift=0.0cm,
            anchor=north west,    
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            ytick={1,2,3,4,5},
            yticklabels={},
            ymin = 0.75, ymax = 5.25,          
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   2.75, 
            lower quartile  =   3.5,
            median          =   4, 
            upper quartile  =   4,
            upper whisker   =   4.75},
        ] coordinates {(1,5) (1, 2)};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   1, 
            lower quartile  =   2,
            median          =   3, 
            upper quartile  =   4,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   3.75, 
            lower quartile  =   4.5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(4, 3)};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   2, 
            lower quartile  =   3,
            median          =   4, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};      
        
    \end{axis}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            name=thirdplot,
            title=\textbf{Timing},
            at={(secondplot.north east)},
            xshift=0.0cm,
            anchor=north west,      
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            yticklabels={},
            ytick={1,2,3,4,5},
            ymin = 0.75, ymax = 5.25,          
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   2.5, 
            lower quartile  =   4,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(1, 2)};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   1, 
            lower quartile  =   2,
            median          =   3, 
            upper quartile  =   3.5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(4, 4)};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   2, 
            lower quartile  =   3,
            median          =   4, 
            upper quartile  =   4.5,
            upper whisker   =   5},
        ] coordinates {};      
        
    \end{axis}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            at={(mainplot.below south west)},
            title=\textbf{Competence},
            yshift=-1cm,
            anchor=north west,
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            ytick={1,2,3,4,5},
            ymin = 0.75, ymax = 5.25,          
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   4, 
            lower quartile  =   4,
            median          =   4, 
            upper quartile  =   4,
            upper whisker   =   4},
        ] coordinates {(1, 2) (1, 3) (1, 5)};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   2, 
            lower quartile  =   3,
            median          =   4, 
            upper quartile  =   4.5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   4, 
            lower quartile  =   4,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};      
        
    \end{axis}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            title=\textbf{Safety},
            at={(secondplot.below south west)},
            yshift=-1cm,
            anchor=north west,    
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            yticklabels={},
            ytick={1,2,3,4,5},
            ymin = 0.75, ymax = 5.25,          
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   4, 
            lower quartile  =   4.5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   3, 
            lower quartile  =   4,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(5, 4)};      
        
    \end{axis}
    \begin{axis}[
            % enlarge x limits=true,
            % enlarge y limits=true,
            title=\textbf{Predictability},
            at={(thirdplot.below south west)},
            yshift=-1cm,
            anchor=north west,   
            width = 0.235\textwidth,
            height = 0.235\textwidth,
            boxplot/draw direction=y,
            xtick={1.5, 4.5},
            xticklabels={Robot, Human},
            yticklabels={},
            ymin = 0.75, ymax = 5.25,
         ]     
         
        \addplot [solid, blue, mark=*, boxplot prepared={
            lower whisker   =   3, 
            lower quartile  =   3.5,
            median          =   4, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, red, mark=*, boxplot prepared={
            lower whisker   =   1, 
            lower quartile  =   2,
            median          =   3, 
            upper quartile  =   4,
            upper whisker   =   5},
        ] coordinates {};
        
        \addplot [solid, blue, mark=*, boxplot prepared={draw position=4,
            lower whisker   =   5, 
            lower quartile  =   5,
            median          =   5, 
            upper quartile  =   5,
            upper whisker   =   5},
        ] coordinates {(4, 4)};
        
        \addplot [solid, red, mark=*, boxplot prepared={draw position=5,
            lower whisker   =   3.25, 
            lower quartile  =   4,
            median          =   4, 
            upper quartile  =   4.5,
            upper whisker   =   5},
        ] coordinates {(5, 3)};      
        
    \end{axis}
    
    
\end{tikzpicture}

